Supersymmetric Completion of an R^2 Term in Five-Dimensional Supergravity

We analyze the structure of a particular higher derivative correction of five-dimensional ungauged and gauged supergravity with eight supercharges. Specifically, we determine all the purely bosonic terms which are connected by the supersymmetry transformation to the mixed gauge-gravitational Chern-Simons term, W wedge tr R wedge R. Our construction utilizes the superconformal formulation of supergravity. As an application, we determine the condition for the supersymmetric anti-de Sitter vacuum with this term. We check that it gives precisely the same condition as the a-maximization in four-dimensional superconformal field theory on the boundary, as predicted by the AdS/CFT correspondence.

==> bib.tex <==

    \bibitem{GST1}

  M.~G\"unaydin, G.~Sierra and P.~K.~Townsend,
  ``The Geometry of $N=2$ Maxwell-Einstein Supergravity and Jordan Algebras,''
 {\slshape   Nucl.\ Phys.\ B }{\bf 242} (1984) 244.
  %%CITATION = NUPHA,B242,244;%%
 

    \bibitem{GST2}

  M.~G\"unaydin, G.~Sierra and P.~K.~Townsend,
  ``Gauging the D = 5 Maxwell-Einstein Supergravity Theories: More on Jordan
  Algebras,''
 {\slshape   Nucl.\ Phys.\ B }{\bf 253} (1985) 573.
  %%CITATION = NUPHA,B253,573;%%
 

    \bibitem{BR}

  E.~Bergshoeff and M.~Rakowski,
  ``An Off-Shell Superspace $R^2$ Action in Six-Dimensions,''
 {\slshape   Phys.\ Lett.\ B }{\bf 191} (1987) 399.
  %%CITATION = PHLTA,B191,399;%%
 

    \bibitem{MoReview}

  T.~Mohaupt,
  ``Black hole entropy, special geometry and strings,''
 {\slshape   Fortsch.\ Phys.\  }{\bf 49} (2001) 3
  [arXiv:hep-th/0007195].
  %%CITATION = HEP-TH 0007195;%%
 

    \bibitem{KO}

  T.~Kugo and K.~Ohashi,
  ``Supergravity tensor calculus in 5D from 6D,''
 {\slshape   Prog.\ Theor.\ Phys.\  }{\bf 104} (2000) 835
  [arXiv:hep-ph/0006231].
  %%CITATION = HEP-PH 0006231;%%
 

    \bibitem{FO}

  T.~Fujita and K.~Ohashi,
  ``Superconformal tensor calculus in five dimensions,''
 {\slshape   Prog.\ Theor.\ Phys.\  }{\bf 106} (2001) 221
  [arXiv:hep-th/0104130].
  %%CITATION = HEP-TH 0104130;%%
 

    \bibitem{Berg0}

  E.~Bergshoeff, S.~Cucu, M.~Derix, T.~de Wit, R.~Halbersma and A.~Van Proeyen,
  ``Weyl multiplets of $N$ = 2 conformal supergravity in five dimensions,''
 {\slshape   JHEP }{\bf 0106} (2001) 051
  [arXiv:hep-th/0104113].
  %%CITATION = HEP-TH 0104113;%%
 

    \bibitem{Berg1}

  E.~Bergshoeff, S.~Cucu, T.~de Wit, J.~Gheerardyn, S.~Vandoren and A.~Van Proeyen,
  ``N = 2 supergravity in five dimensions revisited,''
 {\slshape   Class.\ Quant.\ Grav.\  }{\bf 21} (2004) 3015
  [Class.\ Quant.\ Grav.\  {\bf 23} (2006) 7149]
  [arXiv:hep-th/0403045].
  %%CITATION = HEP-TH 0403045;%%
 

    \bibitem{Ferrara1}

  S.~Ferrara, R.~R.~Khuri and R.~Minasian,
  ``M-Theory on a Calabi-Yau Manifold,''
 {\slshape   Phys.\ Lett.\ B }{\bf 375} (1996) 81
  [arXiv:hep-th/9602102].
  %%CITATION = HEP-TH 9602102;%%
 

    \bibitem{Ferrara2}

  I.~Antoniadis, S.~Ferrara, R.~Minasian and K.~S.~Narain,
  ``$ R^4$ couplings in M- and type II theories on Calabi-Yau spaces,''
 {\slshape   Nucl.\ Phys.\ B }{\bf 507} (1997) 571
  [arXiv:hep-th/9707013].
  %%CITATION = HEP-TH 9707013;%%
 

    \bibitem{veryspecial}

  B.~de Wit and A.~Van Proeyen,
  ``Broken Sigma Model Isometries in Very Special Geometry,''
 {\slshape   Phys.\ Lett.\ B }{\bf 293} (1992) 94
  [arXiv:hep-th/9207091].
  %%CITATION = HEP-TH 9207091;%%
 

    \bibitem{interpretation-of-higher}

  D.~A.~Eliezer and R.~P.~Woodard,
  ``The Problem of Nonlocality in String Theory,''
 {\slshape   Nucl.\ Phys.\ B }{\bf 325} (1989) 389.
  %%CITATION = NUPHA,B325,389;%%
 

    \bibitem{interpretation-of-higher2}

  T.~C.~Cheng, P.~M.~Ho and M.~C.~Yeh,
  ``Perturbative approach to higher derivative and nonlocal theories,''
 {\slshape   Nucl.\ Phys.\ B }{\bf 625} (2002) 151
  [arXiv:hep-th/0111160].
  %%CITATION = HEP-TH 0111160;%%
 

    \bibitem{aux-elimination}

  P.~C.~Argyres, A.~M.~Awad, G.~A.~Braun and F.~P.~Esposito,
  ``Higher-derivative terms in $N$ = 2 supersymmetric effective actions,''
 {\slshape   JHEP }{\bf 0307} (2003) 060
  [arXiv:hep-th/0306118].
  %%CITATION = HEP-TH 0306118;%%
 

    \bibitem{5dgaugedattractor}

  A.~Chou, R.~Kallosh, J.~Rahmfeld, S.~J.~Rey, M.~Shmakova and W.~K.~Wong,
  ``Critical points and phase transitions in 5d compactifications of
  M-theory,''
 {\slshape   Nucl.\ Phys.\ B }{\bf 508} (1997) 147
  [arXiv:hep-th/9704142].
  %%CITATION = HEP-TH 9704142;%%
 

    \bibitem{IW}

  K.~Intriligator and B.~Wecht,
  ``The exact superconformal R-symmetry maximizes $a$,''
 {\slshape   Nucl.\ Phys.\ B }{\bf 667} (2003) 183
  [arXiv:hep-th/0304128].
  %%CITATION = HEP-TH 0304128;%%
 

    \bibitem{adsamax}

  Y.~Tachikawa,
  ``Five-dimensional supergravity dual of $a$-maximization,''
 {\slshape   Nucl.\ Phys.\ B }{\bf 733} (2006) 188
  [arXiv:hep-th/0507057].
  %%CITATION = HEP-TH 0507057;%%
 

    \bibitem{currentcorrelator}

  E.~Barnes, E.~Gorbatov, K.~Intriligator and J.~Wright,
  ``Current correlators and AdS/CFT geometry,''
 {\slshape   Nucl.\ Phys.\ B }{\bf 732} (2006) 89
  [arXiv:hep-th/0507146].
  %%CITATION = HEP-TH 0507146;%%
 

    \bibitem{AW}

  L.~Alvarez-Gaum\'e and E.~Witten,
  ``Gravitational Anomalies,''
 {\slshape   Nucl.\ Phys.\ B }{\bf 234} (1984) 269.
  %%CITATION = NUPHA,B234,269;%%
 

    \bibitem{ON}

  S.~Nojiri and S.~D.~Odintsov,
  ``On the conformal anomaly from higher derivative gravity in AdS/CFT
  correspondence,''
 {\slshape   Int.\ J.\ Mod.\ Phys.\ A }{\bf 15} (2000) 413
  [arXiv:hep-th/9903033].
  %%CITATION = HEP-TH 9903033;%%
 

    \bibitem{GN}

  M.~Blau, K.~S.~Narain and E.~Gava,
  ``On subleading contributions to the AdS/CFT trace anomaly,''
 {\slshape   JHEP }{\bf 9909} (1999) 018
  [arXiv:hep-th/9904179].
  %%CITATION = HEP-TH 9904179;%%
 

    \bibitem{FMS}

  M.~Fukuma, S.~Matsuura and T.~Sakai,
  ``Higher-derivative gravity and the AdS/CFT correspondence,''
 {\slshape   Prog.\ Theor.\ Phys.\  }{\bf 105} (2001) 1017
  [arXiv:hep-th/0103187].
  %%CITATION = HEP-TH 0103187;%%
 

